First-order phase transition and the equation of state in a 2D granular fluid

We present experimental evidence for a first-order freezing/melting phase transition in a nonequilibrium system -- an oscillated two-dimensional isobaric granular fluid. The steady-state transition occurs between a gas and a crystal and is characterized by a discontinuous change in both density and temperature. It is suppressed if the number of particles is incommensurate with the cell size, shows rate-dependent hysteresis, and obeys the Lindemann criterion for melting. Further, the measured equation of state both above and below the phase transition compares well with theory.

==> macros.tex <==
%math stuff

\newcommand{\Vect}[1]{\mbox{\boldmath\bf #1\unboldmath}}  
\newcommand{\unitvector}[1]{\mbox{$\widehat{#1}$}}  
\newcommand{\function}[2]{\mbox{#1$(#2)$}}  
\newcommand{\abs}[1]{\mbox{$\left| \mbox{\ensuremath{#1}} \right|$}}   
\newcommand{\derivative}[3]{\mbox{${\displaystyle \frac{#1#2}{#1#3}}$}}  
\newcommand{\nderivative}[4]{\mbox{${\displaystyle 
	\frac{{#2}^{#1}#3}{{#2#4}^{#1}}}$}}  
\newcommand{\Exp}[1]{\mbox{$\exp\left({\displaystyle #1}\right) $}} 
\newcommand{\vectorcomp}[2]{\sub{#1}{#2}}  
\newcommand{\tint}{{\displaystyle \int\!\!\!\!\int\!\!\!\!\int}}
\newcommand{\dint}{{\displaystyle \int\!\!\!\!\int}}
\newcommand{\sint}{{\displaystyle \int}}
\newcommand{\Tensor}[1]{\mbox{\bf\sf#1}}
\newcommand{\complex}[1]{\mbox{\sl\sf#1}}
\newcommand{\Complex}[1]{\magnitude{#1}\Exp{\I\Phase{#1}}}
\newcommand{\CComplex}[1]{\magnitude{#1}\Exp{-\I\Phase{#1}}}
\newcommand{\COmplex}[2]{\magnitude{#1}\Exp{#2}}
\newcommand{\CCOmplex}[2]{\magnitude{#1}\Exp{-#2}}
\newcommand{\magnitude}[1]{\script{#1}}
\newcommand{\COMPLEX}[2]{{#1}\Exp{#2}}
\newcommand{\CCOMPLEX}[2]{{#1}\Exp{-#2}}
\newcommand{\Phase}[1]{\mbox{$\phase_{#1}$}}
\newcommand{\IM}{\mbox{Im}}
\newcommand{\RE}{\mbox{Re}}
\newcommand{\Grad}[1]{\mbox{$\Vect{$\nabla$}\!#1$}}
\newcommand{\Laplacian}[1]{\mbox{$\nabla^2\,#1$}}
\newcommand{\Div}[1]{\mbox{$\Vect{$\nabla$} \cdot #1$}}
\newcommand{\Curl}[1]{\mbox{$\Vect{$\nabla$} \times #1$}}
\newcommand{\CC}[1]{\mbox{$#1^{*}$}}
\newcommand{\trans}[1]{#1$^{\prime}$}
\newcommand{\order}[1]{\mbox{${\cal O}\left(#1\right)$}}
\newcommand{\dirac}[1]{\mbox{$\delta(#1)$}}
\newcommand{\Kron}[2]{\mbox{$\delta_{#1#2}$}}
\newcommand{\altsym}[3]{\mbox{$\epsilon_{#1#2#3}$}}


\newcommand{\e}[1]{\mbox{$\times 10^{#1}$}}
\newcommand{\sn}[2]{\mbox{${#1}\e{{#2}}$}}
\newcommand{\area}{{\it A}}
\newcommand{\surface}{\sigma}
\newcommand{\pos}{r}
\newcommand{\conpos}{k}
\newcommand{\vel}{v}
\newcommand{\cvel}{u}
\newcommand{\force}{F}
\newcommand{\convel}{q}
\newcommand{\dacc}{a}
\newcommand{\gen}{R}
\newcommand{\congen}{K}
\newcommand{\vol}{V}
\newcommand{\energy}{U}
\newcommand{\ang}{\alpha}
\newcommand{\phase}{\Phi}
\newcommand{\dV}{{\it \,dV}}
\newcommand{\I}{{\it i\,}}

% mri stuff

\newcommand{\alphapulse}[1]{\mbox{$#1$--pulse}}  
\newcommand{\alphapulses}[1]{\mbox{$#1$--pulses}}  
\newcommand{\pipulse}{\alphapulse{\pi}}  
\newcommand{\pipulses}{\alphapulses{\pi}}  
\newcommand{\pihalfpulse}{\alphapulse{\frac{\pi}{2}}}
\newcommand{\pihalfpulses}{\alphapulses{\frac{\pi}{2}}}
\newcommand{\freq}{\mbox{$\omega$}}
\newcommand{\Cfreq}{\mbox{$\Omega$}}
\newcommand{\MCfreq}{\mbox{${\sl\Omega}$}}
\newcommand{\larmorfreq}{\mbox{$\freq_L$}}  
\newcommand{\mass}{\mbox{\it m}}
\newcommand{\charge}{\mbox{\it e}}
\newcommand{\J}{J}
\newcommand{\angmoment}{L}
\newcommand{\torque}{N}
\newcommand{\magmoment}{m}
\newcommand{\magn}{M}
\newcommand{\magG}{G}
\newcommand{\fmagG}{\mbox{$\Gamma$}}
\newcommand{\magf}{H}
\newcommand{\magi}{B}
\newcommand{\magpot}{A}
\newcommand{\Mperm}{\mbox{$\mu$}}
\newcommand{\Msuscep}{\mbox{$\chi_m$}}
\newcommand{\relaxation}{\mbox{\it T}}
\newcommand{\Ttwostar}{\mbox{${\relaxation_2}^{*}$}}
\newcommand{\signal}{\mbox{\it S}}
\newcommand{\tmag}{\mbox{$\Vect{\magn}_T$}}  
\newcommand{\gyro}{\mbox{$\gamma$}}
\newcommand{\reptime}{\mbox{$T_r$}}
\newcommand{\te}{\mbox{$T_e$}}

% misc stuff

\newcommand{\fig}{\begin{figure}}
\newcommand{\efig}{\end{figure}}
\newcommand{\figsref}[2]{Fig. \ref{#1}-\ref{#2}}
\newcommand{\Figsref}[2]{Figure \ref{#1}-\ref{#2}}
\newcommand{\figref}[1]{Fig. \ref{#1}}
\newcommand{\Figref}[1]{Figure \ref{#1}}
\newcommand{\subfigref}[2]{Fig. \ref{#1}(#2)}
\newcommand{\Subfigref}[2]{Figure \ref{#1}(#2)}
\newcommand{\Table}{\begin{table}}  
\newcommand{\etable}{\end{table}}  
\newcommand{\eq}{\begin{equation}}  
\newcommand{\eeq}{\end{equation}}  
\newcommand{\eqa}{\begin{eqnarray}}  
\newcommand{\eeqa}{\end{eqnarray}}  
\newcommand{\eqref}[1]{(\ref{eq:#1})}
\newcommand{\eqsref}[2]{(\ref{eq:#1}--\ref{eq:#2})}
\newcommand{\Eqref}[1]{Equation (\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations (\ref{eq:#1}--\ref{eq:#2})}
\newcommand{\tableref}[1]{table \ref{#1}}
\newcommand{\Tableref}[1]{Table \ref{#1}}
\newcommand{\secref}[1]{(\S\,\ref{#1})}
\newcommand{\secsref}[2]{(\S\,\ref{#1}--\ref{#2})}
\newcommand{\Secref}[1]{Section \ref{#1}}
\newcommand{\Secsref}[2]{Sections \ref{#1}--\ref{#2}}
\newcommand{\chapref}[1]{chapter \ref{c:#1}}
\newcommand{\Chapref}[1]{Chapter \ref{c:#1}}
\newcommand{\partref}[1]{part \ref{p:#1}}
\newcommand{\Partref}[1]{Part \ref{p:#1}}
\newcommand{\appref}[1]{appendix \ref{a:#1}}
\newcommand{\Appref}[1]{Appendix \ref{a:#1}}
\newcommand{\noteref}[3]{#1\ref{#2}#3}
\newcommand{\script}[1]{\mbox{${\cal #1}$}}
\newcommand{\sub}[2]{\mbox{${\mbox{#1}}_{#2}$}}  
\newcommand{\asub}[3]{\begin{array}[#1]{c}{#2}\\{#3}\end{array}}
\newcommand{\zbox}[1]{\makebox[0mm][c]{#1}}
\newcommand{\mword}[1]{\mbox{#1}}
\newcommand{\smword}[1]{\mbox{\protect\scriptsize#1}}
\newcommand{\rem}[1]{[{\it remark: #1}]}
\newenvironment{remlist}{\it remarks:
	\begin{itemize} \it}{\end{itemize}}
% create hanging indents
\newcommand{\newitem}[2]{\hangafter=1 \hangindent=5cm \noindent
			{\bf #1} \hspace{.375cm}
			\parbox[t]{\textwidth}{#2}
			\vspace{.25cm}}

% constants

\newcommand{\Ma}{\mbox{\it Ma}}
\newcommand{\Pran}{\mbox{\it Pr}}
\newcommand{\Da}{\mbox{\it Da}}
\newcommand{\Rey}{\mbox{\it Re}}
\newcommand{\Ra}{\mbox{\it Ra}}
\newcommand{\Rac}{\mbox{$\Ra_c$}}
\newcommand{\ra}{\mbox{$\epsilon$}}
\newcommand{\Tc}{\mbox{$\tempdiff_c$}}
\newcommand{\vdiff}{\mbox{$\tau_v$}}
\newcommand{\hdiff}{\mbox{$\tau_h$}}
\newcommand{\Vrev}{\mbox{$\vol_{\smword{rev}}$}}
\newcommand{\Nu}{\mbox{\it Nu}}
\newcommand{\shockangle}{\mbox{$\beta$}}
\newcommand{\wedgeangle}{\mbox{$\Theta$}}
\newcommand{\cellheight}{\mbox{\it h}}
\newcommand{\sandwichheight}{\mbox{\it H}}
\newcommand{\cellwidth}{\mbox{\it W}}
\newcommand{\celllength}{\mbox{\it L}}
\newcommand{\lengthscale}{\mbox{\it L}}
\newcommand{\beadsize}{\mbox{\it d}}
\newcommand{\porescale}{\mbox{$\delta$}}
\newcommand{\gravity}{\mbox{$g$}}
\newcommand{\wavelength}{\mbox{$\lambda$}}
\newcommand{\wavenumber}{\mbox{\it q}}
\newcommand{\rwavenumber}{\mbox{\it Q}}
\newcommand{\aspect}{\mbox{$\Gamma$}}
\newcommand{\Is}{\mbox{$\mword{I}_{\smword{s}}$}}
\newcommand{\rest}{\mbox{$\epsilon$}}
\newcommand{\acc}{\mbox{$\Gamma$}}
\newcommand{\accc}{\mbox{$\acc_c$}}
\newcommand{\damp}{\mbox{$A$}}
\newcommand{\partdia}{\mbox{$\sigma$}}
\newcommand{\dfreq}{\mbox{$f$}}
\newcommand{\ndfreq}{\mbox{$f_0$}}
\newcommand{\stress}{\mbox{$\tau$}}
\newcommand{\strain}{\mbox{$\gamma$}}
\newcommand{\strainrate}{\mbox{$\dot{\strain}$}}

% fluid stuff

\newcommand{\heatflowratio}{\mbox{$\Lambda$}}
\newcommand{\heatflow}{\mbox{\it Q}}
\newcommand{\heatflux}{\mbox{\it q}}
\newcommand{\expansion}{\mbox{$\beta$}}
\newcommand{\specheat}{\mbox{\it c}}
\newcommand{\heatratio}{\mbox{$\sigma$}}
\newcommand{\conductivity}{\mbox{\it k}}
\newcommand{\porosity}{\mbox{$\phi$}}
\newcommand{\volumefrac}{\mbox{$\nu$}}
\newcommand{\ivelocity}{\mbox{V}}
\newcommand{\fvelocity}{\mbox{v}}
\newcommand{\temp}{\mbox{\it T}}
\newcommand{\granT}{\mbox{T}}
\newcommand{\tempdiff}{\mbox{$\Delta\temp$}}
\newcommand{\dfvelocity}{\mbox{u}}
\newcommand{\dtemp}{\mbox{$\theta$}}
\newcommand{\pressure}{\mbox{\it P}}
\newcommand{\density}{\mbox{$\rho$}}
\newcommand{\dviscosity}{\mbox{$\eta$}}
\newcommand{\kviscosity}{\mbox{$\nu$}}
\newcommand{\shearviscosity}{\mbox{$\mu$}}
\newcommand{\bulkviscosity}{\mbox{$\lambda$}}
\newcommand{\diffusivity}{\mbox{$\alpha$}}
\newcommand{\permeability}{\mbox{K}}
\newcommand{\accelcoeff}{\mbox{\it a}}
\newcommand{\daccelcoeff}{\mbox{\it A}}
\newcommand{\vorticity}{\mbox{$\xi$}}


% acronyms

\newcommand{\PMC}{\mbox{PMC}}
\newcommand{\RBC}{\mbox{RBC}}
\newcommand{\MRI}{\mbox{MRI}}
\newcommand{\GRE}{\mbox{GRE}}
\newcommand{\EPI}{\mbox{EPI}}
\newcommand{\SE}{\mbox{SE}}
\newcommand{\FSE}{\mbox{FSE}}
\newcommand{\NMR}{\mbox{NMR}}
\newcommand{\SNR}{\mbox{SNR}}
\newcommand{\hcp}{\mbox{h.c.p.}}
\newcommand{\rf}{\mbox{r.f.}}
\newcommand{\rev}{\mbox{r.e.v.}}
\newcommand{\fid}{\mbox{f.i.d.}}
\newcommand{\dfft}{\mbox{DFFT}}
\newcommand{\fft}{\mbox{FFT}}

% units

\newcommand{\WpercmperK}{\nobreak\mbox{$\;$W\,cm$^{-1}$\,K$^{-1}$}}
\newcommand{\JpergperK}{\nobreak\mbox{$\;$J\,g$^{-1}$\,K$^{-1}$}}
\newcommand{\Gpercm}{\nobreak\mbox{$\;$G\,cm$^{-1}$}}
\newcommand{\Gpers}{\nobreak\mbox{$\;$G\,s$^{-1}$}}
\newcommand{\gpercc}{\nobreak\mbox{$\;$g\,cm$^{-3}$}}
\newcommand{\hzperT}{\nobreak\mbox{$\;$Hz\,T$^{-1}$}}
\newcommand{\s}{\nobreak\mbox{$\;$s}}
\newcommand{\ms}{\nobreak\mbox{$\;$ms}}
\newcommand{\us}{\nobreak\mbox{$\;\mu$s}}
\newcommand{\mins}{\nobreak\mbox{$\;$min}}
\newcommand{\hrs}{\nobreak\mbox{$\;$hrs}}
\newcommand{\days}{\nobreak\mbox{$\;$days}}
\newcommand{\years}{\nobreak\mbox{$\;$years}}
\newcommand{\inch}{\nobreak\mbox{$\;$in}}
\newcommand{\cm}{\nobreak\mbox{$\;$cm}}
\newcommand{\mm}{\nobreak\mbox{$\;$mm}}
\newcommand{\um}{\nobreak\mbox{$\;\mu$m}}
\newcommand{\mmpers}{\nobreak\mbox{$\;$mm\,s$^{-1}$}}
\newcommand{\cmpers}{\nobreak\mbox{$\;$cm\,s$^{-1}$}}
\newcommand{\cmpersqs}{\nobreak\mbox{$\;$cm\,s$^{-2}$}}
\newcommand{\ccpers}{\nobreak\mbox{$\;$cm$^{3}$\,s$^{-1}$}}
\newcommand{\umpers}{\nobreak\mbox{$\;\mu$m\,s$^{-1}$}}
\newcommand{\cmsqpers}{\nobreak\mbox{$\;$cm$^2$\,s$^{-1}$}}
\newcommand{\spercm}{\nobreak\mbox{$\;$s\,cm$^{-1}$}}
\newcommand{\K}{\nobreak\mbox{$\;$K}}
\newcommand{\mK}{\nobreak\mbox{$\;$mK}}
\newcommand{\degrees}{\nobreak\mbox{$\;^\circ$C}}
\newcommand{\C}{\nobreak\mbox{$\;^\circ$C}}
\newcommand{\T}{\nobreak\mbox{$\;$T}}
\newcommand{\mhz}{\nobreak\mbox{$\;$MHz}}
\newcommand{\hz}{\nobreak\mbox{$\;$Hz}}
\newcommand{\fps}{\nobreak\mbox{$\;$fps}}
\newcommand{\radpers}{\nobreak\mbox{$\;$rad\,s$^{-1}$}}
\newcommand{\molar}{\nobreak\mbox{$\;$M}}
\newcommand{\period}{\nobreak\mbox{$\;$T}}









